Uncovering the Impact of Chain-of-Thought Reasoning for Direct Preference Optimization: Lessons from Text-to-SQL

Direct Preference Optimization (DPO) has proven effective in complex reasoning tasks like math word problems and code generation. However, when applied to Text-to-SQL datasets, it often fails to improve performance and can even degrade it. Our investigation reveals the root cause: unlike math and code tasks, which naturally integrate Chain-of-Thought (CoT) reasoning with DPO, Text-to-SQL datasets typically include only final answers (gold SQL queries) without detailed CoT solutions. By augmenting Text-to-SQL datasets with synthetic CoT solutions, we achieve, for the first time, consistent and significant performance improvements using DPO. Our analysis shows that CoT reasoning is crucial for unlocking DPO's potential, as it mitigates reward hacking, strengthens discriminative capabilities, and improves scalability. These findings offer valuable insights for building more robust Text-to-SQL models. To support further research, we publicly release the code and CoT-enhanced datasets.

==> DPO.tex <==
%\textbf{Learning Objective}

\subsection{Learning Objective}

For Reinforcement Learning with Human Feedback (RLHF) incorporating KL penalty, the learning objective is defined as \citep{ouyang2022rlhf}:
%\begin{adjustbox}{max width=\textwidth}
\begin{align*}
\max_{\pi_{\theta}}\mathbb{E}_{x\sim\mathcal{D},y\sim\pi_{\theta}(y|x)} & \left[r_{\phi}(x,y)\right] \\
 -\beta\mathbb{D}_{\mathrm{KL}} & \left[\pi_{\theta}(y\mid x)\mid\mid\pi_{\mathrm{ref}}(y\mid x)\right]
\end{align*}
%\end{adjustbox}

Here, $\pi_{\mathrm{ref}}$ and $\pi_{\theta}$ represent the initial model distribution and the optimized policy, respectively, while $r_{\phi}$ denotes a parameterized reward model.

Direct Preference Optimization (DPO) reformulates the objective by replacing the reward function with a differentiable form, reflecting the relationship between the optimal policy and the reward function. This leads to a new objective:
%$$\mathcal{L}_{\mathrm{DPO}}(\pi_{\theta};\pi_{\mathrm{ref}})=$$
%\resizebox{\linewidth}{!}{}
%\begin{adjustbox}{max width=\textwidth}
%\begin{align*}
%$$\mathbb{E}_{(x,y_{w},y_{l})\sim\mathcal{D}}\left[\log \sigma\left(\beta\log\frac{\pi_{\theta}(y_{w}\mid x)}{\pi_{\mathrm{ref}}(y_{w}\mid x)}
%-\beta\log\frac{\pi_{\theta}(y_{l}\mid x)}{\pi_{\mathrm{ref}}(y_{l}\mid x)}\right )\right ]$$
%\end{align*}
%\end{adjustbox}
\begin{align*}
\mathbb{E}_{(x,y_{w},y_{l})\sim\mathcal{D}}\left[\log \sigma\left(\beta \log\frac{\pi_{\theta}(y_{w}\mid x)}{\pi_{\mathrm{ref}}(y_{w}\mid x)}\right.\right. \\
\left.\left.  -\beta\log\frac{\pi_{\theta}(y_{l}\mid x)}{\pi_{\mathrm{ref}}(y_{l}\mid x)} \right)\right]
\end{align*}


In this formulation, $y_w$ denotes the chosen output and $y_l$ denotes the rejected output. The parameter $\beta$ controls the penalty strength imposed by the KL divergence. By collecting pairwise preference data, the model can be optimized using supervised fine-tuning, achieving a performance comparable to RLHF \citep{rafailov2024dpo}.

\subsection{Implicit Reward}
%\textbf{Implicit Reward}

DPO implicitly encodes a reward model within the generative model. The reward of a given input-output pair $(x, y)$ can be derived as:

$$r_{\theta}(x, y) = \beta \log \frac{\pi_\theta(y\mid x)}{\pi_{\mathrm{ref}}(y\mid x)}$$

As the DPO training progresses, the optimized model simultaneously becomes a better generative model and a more refined reward model. After training, the implicit reward model, which is derived via conditional likelihood, can be independently used as a reward function \citep{lambert2024rewardbench, chen2024bootstrappinglanguagemodelsdpo}.

%\textbf{Credit Assignment}
\subsection{Credit Assignment}

The implicit reward scores the entire output as a whole. By decomposing the conditional probability that featuring autoregressive generation process, the reward can be re-expressed as:
$$r_{\theta}(x,y) = \sum_{t=1}^{T}\beta \log \frac{\pi_\theta(y_t\mid x,y_{1:t-1})}{\pi_{\mathrm{ref}}(y_t\mid x,y_{1:t-1})}$$

This decomposition allows for the calculation of token-level rewards, as the model score for each token can be identified separately. Although DPO training uses supervision at the full-sequence level, evidence has shown that the model can generalize compositionality to some extent, allowing it to distribute the reward signal to key tokens \citep{rafailov2024dpo2}. This facilitates credit assignment across the output sequence. The resulting dense reward can be utilized for further training and optimization \citep{zhong2024dpo-ppo}.



==> Tables/ErrorAnalysis-bk.tex <==
\definecolor{darkgreen}{RGB}{0,150,0}
\begin{table*}[t]
\centering
%\setlength{\tabcolsep}{5pt} % Adjust column padding
%\renewcommand{\arraystretch}{1.3} % Adjust row spacing
%\begin{tabularx}{\textwidth}{lXlccc}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c p{3.5cm} l | c | c | c | c | c | c}
\toprule
\textbf{Category} & \textbf{Description} & \textbf{Type} & \multicolumn{2}{c}{\makecell{\textbf{Vanilla DPO} \\ \textbf{Fix (\%)}}} \vline & \multicolumn{2}{c}{\makecell{\textbf{Syn CoT DPO} \\ \textbf{Fix (\%)}}} \vline & \multicolumn{2}{c}{\textbf{\textbf{$\Delta$(\%)}}} \\
\midrule
\multirow{1}{*}{External Knowledge} 
    & Neglect of hints
    & \textbf{[A1] EK} 
    & 0.0 (0/3)
    & 0.0 (0/3) 
    & 37.5 (3/8)
    & \textbf{37.5 (3/8)} 
    & -
    & - \\
\midrule
\multirow{6}{*}{Schema Linking} 
    & \multirow{6}{=}{Fails to match the question with its concerning table and columns}
    & [B1] Table 
    & \multirow{6}{*}{\makecell{15.0 \\ (58/387)}}
    & 13.0 (12/92) 
    & \multirow{6}{*}{\makecell{24.5 \\ (95/388)}}
    & 15.9 (11/69) 
    & \textbf{\textcolor{red}{+2.9}}
    & \multirow{6}{*}{\textbf{\textcolor{red}{+9.5}}}
    \\
    & & \textbf{[B2] JOIN} &
    & 15.6 (12/77) &
    & \textbf{32.1 (18/56)}
    & \textbf{\textcolor{red}{+16.5}} & \\
    & & [B3] Column &
    & 10.3 (7/68) &
    & 16.1 (10/62)
    & \textbf{\textcolor{red}{+5.8}} & \\
    & & \textbf{[B4] Hallucination} &
    & 23.7 (14/59) &
    & \textbf{27.2 (28/102)}
    & \textbf{\textcolor{red}{+3.5}} & \\
    & & [B5] Condition &
    & 16.7 (10/60) &
    & 23.2 (16/69) 
    & \textbf{\textcolor{red}{+6.5}} & \\
    & & \textbf{[B6] NULL/DISTINCT} &
    & 9.7 (3/31) &
    & \textbf{40.0 (12/30)}
    & \textbf{\textcolor{red}{+30.3}} & \\
\midrule
\multirow{2}{*}{Value Retrieval}
    & \multirow{2}{=}{Mismatch of condition with its storage format}
    & [C1] String/Number 
    & \multirow{2}{*}{\makecell{14.6 \\ (7/48)}}
    & 4.5 (1/22) 
    & \multirow{2}{*}{\makecell{26.2 \\ (11/42)}}
    & 21.1 (4/19) 
    & \textbf{\textcolor{red}{+16.6}}
    & \multirow{2}{*}{\textbf{\textcolor{red}{+11.6}}}
    \\
    & & \textbf{[C2] Date} &
    & 23.1 (6/26) &
    & \textbf{30.4 (7/23)}
    & \textbf{\textcolor{red}{+7.3}} & \\
\midrule
\multirow{3}{*}{Operation}
    & \multirow{3}{=}{Misunderstands required operation in the question.}
    & [D1] Mathematical Formula 
    & \multirow{3}{*}{\makecell{8.7 \\ (12/138)}}
    & 13.3 (6/45)
    & \multirow{3}{*}{\makecell{17.2 \\ (23/134)}}
    & 18.2 (8/44) 
    & \textbf{\textcolor{red}{+4.9}}
    & \multirow{3}{*}{\textbf{\textcolor{red}{+8.5}}}
    \\
    & & [D2] Aggregation &
    & 6.7 (5/75) &
    & 18.2 (12/66) 
    & \textbf{\textcolor{red}{+11.5}} & \\
    & & [D3] Complex Operation &
    & 5.6 (1/18) &
    & 12.5 (3/24) 
    & \textbf{\textcolor{red}{+6.9}} & \\
\midrule
\multirow{4}{*}{Information}
    & \multirow{4}{=}{Fails to organize information in the right way}
    & [E1] Redundant/Incomplete 
    & \multirow{4}{*}{\makecell{13.2 \\ (7/53)}}
    & 11.8 (4/34) 
    & \multirow{4}{*}{\makecell{23.4 \\ (11/47)}}
    & 19.2 (5/26) 
    & \textbf{\textcolor{red}{+7.4}}
    & \multirow{4}{*}{\textbf{\textcolor{red}{+10.2}}}
    \\
    & & \textbf{[E2] Column Sequence} &
    & 0 (0/5) &
    & \textbf{42.9 (3/7)}
    & - & \\
    & & [E3] ORDER BY/LIMIT &
    & 9.1 (1/11) &
    & 12.5 (1/8) 
    & \textbf{\textcolor{red}{+3.4}} & \\
    & & \textbf{[E4] Format} &
    & 66.7 (2/3) &
    & \textbf{33.3 (2/6)}
    & - & \\
\midrule
Syntax Error 
    & Inexecutatble SQL 
    & [F1] Syntax 
    & 14.3 (2/14) 
    & 14.3 (2/14) 
    & 13.3 (2/15)
    & 13.3 (2/15)
    & \textbf{\textcolor{darkgreen}{-1.0}}
    & \textbf{\textcolor{darkgreen}{-1.0}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison of Vanilla and Syn CoT DPO correction capability across error types on Bird development set (greedy). The base model is Qwen2.5-7B-Instruct. Fix rate difference is reported if $n>5$ for both models. Error types of which Syn CoT fixes more than $25\%$ in the DPO phase are bolded.}
\label{table:ErrorAnalysis}
\end{table*}

==> Tables/IntroCoT.tex <==
\definecolor{darkgreen}{RGB}{0,150,0}
\begin{table}[h!]
    \centering
\begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{c|c}
    \toprule
       \textbf{Model}  &  \textbf{EX} \\
    \midrule
        Vanilla & 61.4 \\
        CoT & 60.8 (\textcolor{darkgreen}{-0.6}) \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{Performance of SFT Qwen2.5-7B-Instruct on Bird Dev (maj@16). \textbf{Vanilla}: SFT on original Bird Train set; \textbf{CoT}: SFT on synthetic chain-of-thought solution generated by gpt-4o-mini-2024-07-18. }
\end{table}

==> Tables/IntroDPO.tex <==
% additional difference comparison
\definecolor{darkgreen}{RGB}{0,150,0}
\begin{table}[h!]
    \centering
\begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{c|c}
    \toprule
       \textbf{Model}  &  \textbf{EX} \\
    \midrule
        SFT & 61.4 \\
        DPO & 60.6 (\textcolor{darkgreen}{-0.8}) \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{Performance of fine-tuned Qwen2.5-7B-Instruct on Bird Dev (maj@16). }
\end{table}

==> Tables/TrainRobMaj.tex <==
\definecolor{darkgreen}{RGB}{0,150,0}
\begin{table}[h!]
    \centering
\begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{c | c | c c c }
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{SFT} & \multicolumn{3}{c}{\textbf{$\beta$}} \\
    & & $0.05$ & $0.1$ & $0.2$ \\
    \midrule
    Vanilla & 61.4 & 59.9 (\textbf{\textcolor{darkgreen}{-1.5}}) & 60.6 (\textbf{\textcolor{darkgreen}{-0.8}}) & 59.8 (\textbf{\textcolor{darkgreen}{-1.6}})\\
    Syn CoT & 63.0 & 65.2 (\textbf{\textcolor{red}{+2.2}}) & 64.9 (\textbf{\textcolor{red}{+1.9}})& 64.7 (\textbf{\textcolor{red}{+1.7}}) \\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{DPO performance across different $\beta$ values (\textbf{maj@16}). Base model is Qwen2.5-Coder-7B-Instruct.}
\end{table}

==> Tables/TrainRobPass.tex <==
\definecolor{darkgreen}{RGB}{0,150,0}
\begin{table}[h!]
    \centering
\begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{c | c | c c c }
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{SFT} & \multicolumn{3}{c}{\textbf{$\beta$}} \\
    & & $0.05$ & $0.1$ & $0.2$ \\
    \midrule
    Vanilla & 55.1 & 56.0 (\textbf{\textcolor{red}{+0.9}}) & 55.7 (\textbf{\textcolor{red}{+0.6}})& 57.0 (\textbf{\textcolor{red}{+1.9}}) \\
    Syn CoT & 54.8 & 59.2 (\textbf{\textcolor{red}{+4.4}}) & 59.2 (\textbf{\textcolor{red}{+4.4}}) & 59.0 (\textbf{\textcolor{red}{+4.2}})\\
    \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{DPO performance across different $\beta$ values (\textbf{pass@1}). Base model is Qwen2.5-Coder-7B-Instruct.}
\end{table}
